Quasi-Monte Carlo tractability of high dimensional integration over products of simplices

Quasi-Monte Carlo (QMC) methods for high dimensional integrals over unit cubes and products of spheres are well-studied in literature. We study QMC tractability of integrals of functions defined over the product of $m$ copies of the simplex $T^d \subset \mathbb{R}^{d}$. The domain is a tensor product of $m$ reproducing kernel Hilbert spaces defined by `weights' $\gamma_{m,j}$, for $j = 1,2, \ldots, m$. Similar to the results on the unit cube in $m$ dimensions, and the product of $m$ copies of the $d$-dimensional sphere, we prove that strong polynomial tractability holds iff $\limsup_{m \rightarrow \infty} \sum_{j=1}^m \gamma_{m,j} < \infty$ and polynomial tractability holds iff $\limsup_{m \rightarrow \infty} \frac{\sum_{j=1}^m \gamma_{m,j}}{\log(m + 1 )} < \infty$. We also show that weak tractability holds iff $\lim_{m \rightarrow \infty} \frac{\sum_{j=1}^m \gamma_{m,j}}{m} = 0$. The proofs employ Sobolev space techniques and weighted reproducing kernel Hilbert space techniques for the simplex and products of simplices as domain. Properties of orthogonal polynomials on a simplex are also used extensively.

==> newcommandsnotbook.tex <==
% options
\allowdisplaybreaks
%\numberwithin{algorithm}{chapter} % now in bookhead.tex

% Caligraphic letters
\newcommand{\ca}{{\cal A}}
\newcommand{\cd}{{\cal D}}
\newcommand{\ce}{{\cal E}}
\newcommand{\cf}{{\cal F}}
\newcommand{\cg}{{\cal G}}
\newcommand{\ch}{{\cal H}}
\newcommand{\ci}{{\cal I}}
\newcommand{\cj}{{\cal J}}
\newcommand{\cl}{{\cal L}}
\newcommand{\cp}{{\cal P}}
\newcommand{\cu}{{\cal U}}
\newcommand{\cv}{{\cal V}}
\newcommand{\cs}{{\cal S}}
\newcommand{\ct}{{\cal T}}
\newcommand{\cw}{{\cal W}}
\newcommand{\cx}{{\cal X}}


% vectors and components
\newcommand{\mbfx}{\mathbf{x}}
\newcommand{\mbfX}{\mathbf{X}}


\newcommand{\bsa}{\boldsymbol{a}}
\newcommand{\bsb}{\boldsymbol{b}}
\newcommand{\bsc}{\boldsymbol{c}}
\newcommand{\bsm}{\boldsymbol{m}}
\newcommand{\bsu}{\boldsymbol{u}}
\newcommand{\bsx}{\boldsymbol{x}}
\newcommand{\bsy}{\boldsymbol{y}}
\newcommand{\bsz}{\boldsymbol{z}}

\newcommand{\bsA}{\boldsymbol{A}}
\newcommand{\bsB}{\boldsymbol{B}}
\newcommand{\bsC}{\boldsymbol{C}}
\newcommand{\bsT}{\boldsymbol{T}}
\newcommand{\bsU}{\boldsymbol{U}}
\newcommand{\bsW}{\boldsymbol{W}}
\newcommand{\bsX}{\boldsymbol{X}}
\newcommand{\bsY}{\boldsymbol{Y}}
\newcommand{\bsZ}{\boldsymbol{Z}}

% Sets
\newcommand{\re}{\mathbb{R}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\natu}{\mathbb{N}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\orth}{\mathbb{O}}

% Index subsets
\newcommand{\negu}{{\neg u}}
\newcommand{\glu}{{\!\::\:\!}}
\newcommand{\bsxu}{\bsx_u}
\newcommand{\bsxnu}{\bsx_\negu}
\newcommand{\bsXu}{\bsX_u}
\newcommand{\bsXnu}{\bsX_\negu}
\newcommand{\bsxv}{\bsx_v}
\newcommand{\bsxnv}{\bsx_\negv}
\newcommand{\bsXv}{\bsX_v}
\newcommand{\bsXnv}{\bsX_\negv}

\newcommand{\lra}{\leftrightarrow}
\newcommand{\tran}{\mathsf{T}} % Transpose

\newcommand{\tmod}{\ \mathsf{mod}\ }

\newcommand{\phm}{\phantom{-}}

\newcommand{\ham}{{\cal H}}
\newcommand{\hi}{{\text{high}}}
\newcommand{\lo}{{\text{low}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\newcommand{\ds}{\displaystyle}

\newcommand{\mrd}{\mathrm{d}}
\newcommand{\rd}{\mathrm{\, d}}

\newcommand{\onevec}{\mathbf{1}}
\newcommand{\one}{{\mathbf{1}}}
\newcommand{\strt}[1]{\sqrt{\mathstrut #1}}

\newcommand{\sfrac}[2]{\frac{#1}{\strut#2}}


% operator symbols
\newcommand{\cond}{{\text{cond}}}
\newcommand{\diag}{{\text{diag}}}
\newcommand{\tr}{{\text{tr}}}

\newcommand{\add}{{\text{add}}}
\newcommand{\res}{{\text{res}}}
\newcommand{\two}{{\text{two}}}
\newcommand{\iid}{{\text{iid}}}
\newcommand{\IID}{{\text{IID}}}
\newcommand{\lhs}{{\text{lhs}}}

\newcommand{\asinh}{{\text{asinh}}}

\newcommand{\opt}{{\mathrm{opt}}}
\newcommand{\var}{{\mathrm{Var}}}
\newcommand{\cov}{{\mathrm{Cov}}}
\newcommand{\cor}{{\mathrm{Corr}}}
\newcommand{\vol}{{\mathbf{vol}}}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\wtu}{{\widetilde U}}
\newcommand{\wtx}{{\widetilde X}}
\newcommand{\wtz}{{\widetilde Z}}

\newcommand{\ninv}{{\frac{1}{n}}}
\newcommand{\code}{} % Define a look for code/pseudocode


\newcommand{\deliver}{{\bf deliver}}
\newcommand{\given}{{\bf given}}

%\newtheorem*{note}{Note}
%\newtheorem*{nb}{N.B}

\DeclareMathOperator{\acosh}{arccosh}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\mce}{{\mathcal E}}
\newcommand{\cc}{{\mathcal C}}
\newcommand{\half}{\text{\textonehalf}}

\newcommand{\hrt}{{\heartsuit}}
\newcommand{\dmd}{\diamondsuit}
\newcommand{\clb}{\clubsuit}
\newcommand{\spd}{\spadesuit}

\renewcommand{\emptyset}{\varnothing}
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

% Distributions

\newcommand{\dbeta}{\text{Beta}}
\newcommand{\dbin}{\text{Bin}}
\newcommand{\dchisq}{\chi^2}
\newcommand{\dexp}{\text{Exp}}
\newcommand{\dgam}{\text{Gam}}
\newcommand{\dpoi}{\text{Poi}}
\newcommand{\dmult}{\text{Mult}}
\newcommand{\dweib}{\text{Weib}}
\newcommand{\dt}{\text{t}}
\newcommand{\ddir}{\text{Dir}}

\newcommand{\dpoiproc}{\mathsf{PP}}
\newcommand{\ddirproc}{\mathsf{DP}}

\newcommand{\dnorm}{\mathcal{N}}
\newcommand{\dwish}{\mathcal{W}}
%\newcommand{\dinvwish}{\mathrm{Inv-}\mathcal{W}}
\newcommand{\dinvwish}{\mathcal{W}^{-1}}

\newcommand{\dunif}{\mathbf{U}} % for U 'arbitrary set'
\newcommand{\dustd}{\mathbf{U}} % for U(0,1) and U[0,1)

\newcommand{\qbeta}{\mathrm{qbeta}}

\newcommand{\dbm}{\mathsf{BM}}
\newcommand{\dbb}{\mathsf{BB}}
\newcommand{\dgbm}{\mathsf{GBM}}

% Movable parameter names

\newcommand{\goal}{\mu} % the desired integrand
\newcommand{\e}{{\mathbb{E}}} % expectation
\newcommand{\domx}{{\mathcal{D}}} % domain of x

% method names and similar things
\newcommand{\anti}{{\text{anti}}}
\newcommand{\prop}{{\text{prop}}}
\newcommand{\strat}{{\mathrm{strat}}}
\newcommand{\nopt}{{n\text{--opt}}}
\newcommand{\mis}{{\text{mis}}}


\newcommand{\hk}{{\mathrm{HK}}}
\newcommand{\even}{{\text{E}}}
\newcommand{\odd}{{\text{O}}}

\newcommand{\win}{{\text{W}}}
\newcommand{\bet}{{\text{B}}}

\newcommand{\diff}{{\text{diff}}}
\newcommand{\produ}{{\text{prod}}}
\newcommand{\ratio}{{\text{ratio}}}

% relations

\newcommand{\dotsim}{\stackrel\centerdot\sim}

% new environments

\newenvironment{exerparts}
  { \begin{enumerate}[\quad\bf a)]
    % set spacing between items
    \addtolength{\itemsep}{-.5\baselineskip}
    % set spacing between lines
   \addtolength{\baselineskip}{-.005\baselineskip} }
  { \end{enumerate} }
  
  \newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
%~~~~~~~~~~~~~~~
% Text with quads around it
%~~~~~~~~~~~~~~~
\newcommand{\qtext}[1]{\quad\text{#1}\quad} 
%~~~~~~~~~~~~~~~
% Shorthand for math formatting
%~~~~~~~~~~~~~~~
\newcommand\mbb[1]{\mathbb{#1}}
\newcommand\mbf[1]{\mathbf{#1}}
\def\mc#1{\mathcal{#1}}
\def\mrm#1{\mathrm{#1}}
%~~~~~~~~~~~~~~~
% Common sets
%~~~~~~~~~~~~~~~
\def\reals{\mathbb{R}} % Real number symbol
\def\integers{\mathbb{Z}} % Integer symbol
\def\rationals{\mathbb{Q}} % Rational numbers
\def\naturals{\mathbb{N}} % Natural numbers
\def\complex{\mathbb{C}} % Complex numbers
%~~~~~~~~~~~~~~~
% Common functions
%~~~~~~~~~~~~~~~
\renewcommand{\exp}[1]{\operatorname{exp}\left(#1\right)} % Exponential
\def\indic#1{\mbb{I}\left({#1}\right)} % Indicator function
\providecommand{\argmax}{\mathop\mathrm{arg max}} % Defining math symbols
\providecommand{\argmin}{\mathop\mathrm{arg min}}
\providecommand{\arccos}{\mathop\mathrm{arccos}}
\providecommand{\dom}{\mathop\mathrm{dom}} % Domain
\providecommand{\range}{\mathop\mathrm{range}} % Range
\providecommand{\diag}{\mathop\mathrm{diag}}
\providecommand{\tr}{\mathop\mathrm{tr}}
\providecommand{\abs}{\mathop\mathrm{abs}}
\providecommand{\card}{\mathop\mathrm{card}}
\providecommand{\sign}{\mathop\mathrm{sign}}
\def\rank#1{\mathrm{rank}({#1})}
\def\supp#1{\mathrm{supp}({#1})}
%~~~~~~~~~~~~~~~
% Common probability symbols
%~~~~~~~~~~~~~~~
\def\E{\mathbb{E}} % Expectation symbol
\def\Earg#1{\E\left[{#1}\right]}
\def\Esubarg#1#2{\E_{#1}\left[{#2}\right]}
\def\P{\mathbb{P}} % Probability symbol
\def\Parg#1{\P\left({#1}\right)}
\def\Psubarg#1#2{\P_{#1}\left[{#2}\right]}
\def\Cov{\mrm{Cov}} % Covariance symbol
\def\Covarg#1{\Cov\left[{#1}\right]}
\def\Covsubarg#1#2{\Cov_{#1}\left[{#2}\right]}
\newcommand{\family}{\mathcal{P}} % probability family / statistical model
%~~~~~~~~~~~~~~~
% Distributions
%~~~~~~~~~~~~~~~
\def\Gsn{\mathcal{N}}
\def\Ber{\textnormal{Ber}}
\def\Bin{\textnormal{Bin}}
\def\Unif{\textnormal{Unif}}
\def\Mult{\textnormal{Mult}}
\def\NegMult{\textnormal{NegMult}}
\def\Dir{\textnormal{Dir}}
\def\Bet{\textnormal{Beta}}
\def\Poi{\textnormal{Poi}}
\def\HypGeo{\textnormal{HypGeo}}
\def\GEM{\textnormal{GEM}}
\def\BP{\textnormal{BP}}
\def\DP{\textnormal{DP}}
\def\BeP{\textnormal{BeP}}
\def\Exp{\textnormal{Exp}}
%~~~~~~~~~~~~~~~
% Theorem-like environments
%~~~~~~~~~~~~~~~
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{problem}{Problem}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
% ------------------------------------------------------------------------
\theoremstyle{definition}
\newtheorem{solution}{Solution}



